Light Field Imaging in the Restrictive Object Space based on Flexible Angular Plane

In some applications, the object space of light field imaging system is restrictive, such as industrial and medical endoscopes. If the traditional light field imaging system is used in the restrictive object space (ROS) directly but without any specific considerations, the ROS will lead to severe microlens image distortions and then affects light field decoding, calibration and 3D reconstruction. The light field imaging in restrictive object space (ROS-LF) is complicated but significant. In this paper, we first deduce that the reason of the microlens image deviation is the position variation of the angular plane, then we propose the flexible angular plane for ROS-LF, while in the traditional light field the angular plane always coincides with the main lens plane. Subsequently, we propose the microlens image non-distortion principle for ROS-LF and introduce the ROS-LF imaging principle. We demonstrate that the difference is an aperture constant term between the ROS-LF and traditional light field imaging models. At last, we design a ROS-LF simulated system and calibrate it to verify principles proposed in this paper.

==> refsentences.tex <==

Other parameters can be estimated as follow: $d_f \approx 300mm$, $d_3 \approx 120mm$, $d_2 \approx 2mm$, $d_1 \approx 140mm$. To verify the non-distortion principle of microlens image, two main lenses with different diameters of $D=3.1mm$ and $D=17.8mm$ are used in this paper, as shown in Fig.\ref{fig9(d)} and \ref{fig9(b)}. Since the left side of  (\ref{Q6}) is 0.0133 and the right side is -0.0044 and 0.0325 respectively, which does not meet the non-distortion principle, the distorted microlens images are shown in Fig.\ref{fig9}.


Furthermore, we select the main lens with diameter $D=50.8mm$ and adapt $d_3$ to 20mm, so that the right side of  (\ref{Q6}) is 3.598 to meet the principle of non-distortion, the microlens image without distortion is shown in Fig.\ref{fig9(c)}. The results verify the correctness of the microlens image non-distortion principle proposed in this paper. However, the adjacent microlens images in Fig.\ref{fig9(c)} are not tangent because the f-number matching principle is not met. Then adapt $d_3$ to 120mm, the right side of  (\ref{Q6}) is 0.1150, meeting the microlens image non-distortion principle. At the same time the left side of  (\ref{Q7}) is 92.06, the right sied is 84.00, meeting the f-number matching principle, and the microlens images are shown in Fig.\ref{fig9(d)}. The above experiments show that the microlens image may be distorted when the object space is restrictive. But the distortion can be improved by adjusting the parameters of the light field imaging system. We can obtain undistorted microlens image when the microlens image non-distortion principle is satisfied, even in restrictive object space. The microlens image non-distortion principle and f-number matching principle proposed in this paper can be used to guide the design of ROS-LF imaging system.

For the calibration, a 4×5 checker grid of 6 mm cells was used as calibration board. It is placed about $200 \sim 300mm$ away from the aperture. The decoding was performed using the MATLAB Light Field Toolbox by Dansereau. A two-step calibration method was used for the ROS-LF calibration. The calibration results are detailed in Table \ref{table2}.

For the microlens image distortion in restrictive object space that adversely affects decoding and 3D reconstruction, we defined the flexible angular plane  based on thorough analysis and experiments. Instead of the angular plane fixed to the main-lens plane, the flexible angular plane is determined by the object space.

Further, we proposed a novel ROS-LF model which has an additional aperture constant $H$ compared with the conventional LF, and the parameters was derived using the two step calibration method. The microlens image non-distortion principle and the f-number matching principle are deduced for system design so we can capture regular-shaped, non-distortion and tangent microlens images.












